Constraining Neutrino Interaction Uncertainties for Neutrino Oscillation Measurements at the T2K Experiment

In the context of neutrino oscillation measurements from the T2K experiment, the off-axis near detector ND280 plays a crucial role in constraining the incoming neutrino flux and neutrino-nucleus interaction cross sections. The result is a robust control over systematic uncertainties in the fit of neutrino oscillation parameters to the data at the T2K far detector, Super-Kamiokande. This paper details the methodology and results of these constraints in the context of the latest neutrino oscillation analysis from T2K. It describes how a new neutrino cross-section model and refined flux prediction are parameterized and fit to data in new ND280 event selections. Additionally, this work reports the results of extensive robustness studies, including fits with alternative interaction models, consistency checks against publicly available cross-section measurements, and \textit{p}-value evaluations, to demonstrate the reliability and robustness of our methodology. Finally, we present a sensitivity study demonstrating that the upgraded ND280, with improved acceptance and a lower hadron threshold, may enhance future constraints and further reduce systematic uncertainties in oscillation measurements.

==> commands.tex <==
\newcommand{\pt}{\ensuremath{p_\textrm{T}}\xspace}
\newcommand{\plong}{\ensuremath{p_\textrm{L}}\xspace}
\newcommand{\dat}{\ensuremath{\delta\alpha_\textrm{T}}\xspace}
\newcommand{\dalphat}{\ensuremath{\delta\alpha_\textrm{T}}\xspace}
\newcommand{\dphit}{\ensuremath{\delta\phi_\textrm{T}}\xspace}
\newcommand{\dpt}{\ensuremath{\delta \pt}\xspace}
\newcommand{\dptvect}{\ensuremath{\delta \vec{p}_\textrm{T}}\xspace}
\newcommand{\dplong}{\ensuremath{\delta \plong}\xspace}
\newcommand{\dptt}{\ensuremath{\delta p_\textrm{TT}}\xspace}
\newcommand{\rvline}{\hspace*{-\arraycolsep}\vline\hspace*{-\arraycolsep}}
\newcommand{\evis}{E\ensuremath{_\textrm{vis}}\xspace}
\newcommand{\pmu}{\ensuremath{p_{\mu}}\xspace}
\newcommand{\cosmu}{\ensuremath{\cos{\theta_{\mu}}}\xspace}

\RequirePackage{xspace}


\newcommand{\sfgd}{Super-FGD\xspace}
\newcommand{\hatpc}{HA-TPC\xspace}
\newcommand{\tof}{TOF\xspace}
\newcommand{\sk}{Super-Kamiokande\xspace}
\newcommand{\ndup}{ND280-Upgrade\xspace}

\newcommand{\cczeropizerop}{CC0$\pi$-0$p$-0$\gamma$ }
\newcommand{\cczeropiNp}{CC0$\pi$-N$p$-0$\gamma$ }
\newcommand{\cconepi}{CC1$\pi^+$-0$\gamma$ }
\newcommand{\ccother}{CC-Other-0$\gamma$ }
\newcommand{\ccphoton}{CC-Photon }

\newcommand{\ccotherold}{CC-Other }

\def\thint   {\ensuremath{\textrm \,\theta_{13}}\xspace} 
\def\thatm   {\ensuremath{\textrm \,\theta_{23}}\xspace} 
\def\thsol  {\ensuremath{\textrm \,\theta_{12}}\xspace} 

\def\nunu       {\ensuremath{\nu}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)

%% Generic parenthesis bar e.g. for nu/nubar
\newlength{\parenbarKernelHeight}
\providecommand{\parenbar}[1]{%
    \settoheight{\parenbarKernelHeight}{\ensuremath{#1}}%
    \addtolength{\parenbarKernelHeight}{0pt}
    \llap{\raisebox{\parenbarKernelHeight}{\scalebox{0.5}[0.5]{(}}}%
    \overline{#1}%
    \rlap{\raisebox{\parenbarKernelHeight}{\scalebox{0.5}[0.5]{)}}}%
    %\vphantom{#1}
}

\providecommand{\nuany}{\ensuremath{\hspace{0.5mm}\parenbar{\nu}}\xspace}
\providecommand{\numuany}{\ensuremath{\nuany_\mu}\xspace}
\providecommand{\nueany}{\ensuremath{\nuany_{e}}\xspace}

\usepackage[colorinlistoftodos]{todonotes}
\providecommand{\assign}[1]{\todo[inline,color=magenta]{\underline{Assigned}: #1}}
\providecommand{\sd}[1]{\todo[inline,color=yellow]{Stephen: #1}}
\providecommand{\cirori}[1]{\todo[inline,color=yellow]{Ciro: #1}}
\providecommand{\mba}[1]{\todo[inline,color=cyan]{Margherita: #1}}
\providecommand{\ks}[1]{\todo[inline,color=green]{Kamil: #1}}
\providecommand{\dah}[1]{\todo[inline,color=pink]{Deborah: #1}}
\providecommand{\lm}[1]{\todo[inline,color=orange]{Laura: #1}}
\providecommand{\cw}[1]{\todo[inline,color=red,textcolor=white]{Clarence: #1}}
\providecommand{\td}[1]{\todo[inline,color=violet]{\textcolor{white}{Tristan: #1}}}
\providecommand{\jc}[1]{\todo[inline,color=lime]{{Jaafar: #1}}}
\definecolor{ablightblue}{HTML}{99b6ff}
\providecommand{\ab}[1]{\todo[inline,color=ablightblue]{Adrien: #1}}
\providecommand{\ml}[1]{\todo[inline,color=brown,textcolor=white]{Mitch: #1}}


